Evacuation decisions in response to natural disasters: Insights from a large-scale social media survey

Evacuation in response to natural disasters is a complex process involving multiple decision-makers at the personal, household, community, and government levels. Consequently, many disparate factors influence who evacuates, when, and how to respond to a nearby disaster. In this paper, we leverage a novel method of data collection through social media to explore the evacuation response decisions of people in areas affected by the 2019-2020 Australian bushfires. We explore the validity of this data collection method for generating plausible estimates of evacuation and its ability to supplement cell phone location data using survey responses. Ultimately, we identify several key factors influencing household decisions on evacuation, specifically focusing on the phenomenon of household members evacuating or returning from evacuation at different times.

==> cuttingboard.tex <==
%\subsubsection{Facebook's Gender-Stratified Displacement Map}


%% Shorten and add other work using Cellphone data
 %We articulate specific hypotheses generated by these observed displacement trends below in Section \ref{hypotheses}.


%Facebook's Displacement Maps use aggregated and de-identified data from people using Facebook on their devices who have opted into location history. Displacement is measured in the area affected by a natural disaster that have abrupt changes in their usual movement patterns as a consequence of the crisis, aggregated to a city level. To establish a baseline, Facebook's Displacement Maps first analyze people’s normal movement patterns in the 30-day period before the crisis. Then analyzes movement patterns in the two-week period after the crisis and compare them with the pre-crisis movement patterns. For both time periods, Facebook's Displacement Maps calculates and compares people’s home location and their typical distance traveled away from home. Populations are defined as ``displaced" when they reside at least two kilometers away from their pre-crisis home locations and their typical distance traveled away from the pre-crisis home has doubled. Populations are considered “never displaced” if either of the above conditions is not met and “unknown” if people have not connected to Facebook at least three days in the two-week period after the crisis. Starting on day 15 after the crisis, Facebook's Displacement Maps produce daily updates of the population status to count the number of people displaced and returned, within and across cities, aggregating to a country level when the city count is too low. Populations that were originally classified as displaced are considered “returned” once they are observed for three days in a row less than two kilometers away from their home location.


%Facebook can be accessed from devices with Internet connectivity, such as personal computers, tablets and smartphones. After registering, users can create a profile revealing information about themselves. They can post text, photos and multimedia which is shared with any other users that have agreed to be their "friend", or, with a different privacy setting, with any reader. Users can also use various embedded apps, join common-interest groups, buy and sell items or services on Marketplace, and receive notifications of their Facebook friends' activities and activities of Facebook pages they follow. Facebook claimed that it had more than 2.3 billion monthly active users as of December 2018. (Wikipedia)

% Among Twitter users living in Puerto Rico, we show how many were displaced, the timing and destination of their displacement, and whether they returned. Among Twitter users arriving in Puerto Rico after the disaster, we show the timing and destination of their trips. We find that 8.3% of resident sample relocated during the months after Hurricane Maria and nearly 4% of were still displaced 9 months later.

%Economics of displacement (whose work gets disrupted)
%There is work on the macroeconomic \citep{hallegatteEconomicsNaturalDisasters2010} and microeconimic \citep{xiaoLocalEconomicImpacts2011} effects of natural disasters. \citet{xiaoLocalEconomicImpacts2011}, for example, has shown that the impact of flooding on macroeconomic activity was minimal, but with significant short-term impact on individual income among affected persons. \citet{xiaoBuildingCommunityResiliency2012} showed that there was a strong association between households returning to the disaster location and re-opening of businesses.  We approach these topics in our work by assessing work disruptions due to displacement.


%Crude climate change models predict a mass migration of “climate refugees,” but an emerging literature on environmental migration suggests that most migration will be short-distance and short-duration within existing migration systems

%\subsection{Displacement compared to evacuation}

%Migration decisions are influenced by the severity of disasters \citep{frankenberg2014demography}. A displacement event can last anywhere from days to years, with many choosing to permanently relocate.  Prior work has compared mobility strategies among individuals living in communities which sustained different degrees of damage due to the 2004 Indian Ocean Tsunami \citep{frankenberg2014demography}. Drawing from a recent example of a severe disaster, the authors observed that in 2010 Port-au-Prince, Haiti lost 23\% of its permanent residents following a magnitude 7.0 earthquake struck near that city \citep{frankenberg2014demography}.  

%Typically it is found that cities or regions exposed to natural hazard events which displace populations recover population loss or even see population growth \citep{valeResilientCityHow2005}. Displacement duration's can vary widely within and between disasters. The ability to return depends on support for rebuilding, insurance and other factors. In this work we look primarily at short term (more than 1 night) evacuations and return (within a few months post disaster). 


%\subsection{The demographics indicators of evacuation and short term displacement}

%There is much work around demographic factors associated with short and long-term displacement. \citet{fussell2010race} and others have explored these major issues for Hurricane Katrina; specifically, \citet{fussell2010race} find that Black residents returned at a much slower pace than white residents even after controlling for socioeconomic status. However, further work demonstrated this was likely due to black residents living in areas more severely affected by flooding. \citet{gabe2005hurricane} discusses the major impact of age, disability status and general earnings loss due to Hurricane Katrina.  \citet{gabe2005hurricane}  observe significant effects on children and the elderly (especially loss of community) following Hurricane Katrina.

%Understanding demographic heterogeneity among affected populations can provide necessary context for these disparities, and can better inform policy response to such events in the future.

%\citet{thompsonEvacuationNaturalDisasters2017} categorizes time post disaster from short (1-8 days) to long (7 years) following a disaster. 

%% Where do people go when they evacuate

%There is a strong interest in displacement duration and destination during and after a given disaster event. Hurricane Katrina in 2005 is a well-studied example for these questions \citep{dewaardDisasterLifeCourse2016}. Of particular importance to the short term evacuation and long term displacement is the issue of differential vulnerability \citep{myersSocialVulnerabilityMigration2008}. Heterogeneity within the population and its vulnerability to environmental hazards due to economic, political and social conditions have been examined  \citep{myersSocialVulnerabilityMigration2008}.

%Mechanical characteristics of displacement have also been explored, including relative timing of evacuation decisions  \citep{elliottRaceClassHurricane2006}, comparisons of out-migration \citep{myersSocialVulnerabilityMigration2008} and return migration \citep{fussellRaceSocioeconomicStatus2010} to affected areas, and infill of local areas and neighborhoods \citep{chamlee-wrightThereNoPlace2009,paisPlacesRecoveryMachines2008}. We build on this work by addressing these parameters directly in our survey and providing additional data to explore these topics.

%Under what circumstances do households split up during displacement


%There is a long standing interest in evacuation and displacement of human populations due to disasters in the social science and demographic literature \citep{thompsonEvacuationNaturalDisasters2017}.  Historically, large-scale post-disaster surveys are complicated by the difficulty of reaching people who have been displaced or evacuated following a disaster \citep{frankenberg2014demography}. Recently, new data sources and methods have become available to measure the population properties of evacuation and displacement behavior due to natural disasters; much of this work has focused on social media and modern geo-location data are now able to assist researchers in making inferences on this population in a cost-effective manner. This line of inquiry includes administrative data (e.g. IRS data \citet{fussellRecoveryMigrationCity2014}; Consumer Panel Data \citet{dewaardOutmigrationReturnMigration2020}), geo-location data (e.g. Facebook Disaster Maps; \citet{maas2019facebook}), and social media data (e.g. Twitter; \citet{martinUsingGeotaggedTweets2020} or Facebook Marketing API data; \citet{alexander20}).  We extend this work by leveraging Facebook's platform to build a sampling frame for a population recently affected by a natural disaster (the Australian bushfires of 2019-2020). In this article, we explore methods for drawing displacement- and evacuation-related inferences by comparing a stratified sample of users who opt into providing their geo-location via smart phones (a small subset of Facebook users) and a random sample of comparable users who are predicted to have been in the affected region prior to the disaster. We further employ rejection sampling to provide a final set of respondents who were actually in the disaster zone prior to the bushfire. In conducting this research we partnered with Facebook's Data for Good program, which has already used mobility data to develop an approach that both identifies evacuation/displacement and relocation after disasters to provide real-time information about displacement to non-governmental organizations (NGOs) for disaster relief purposes  \citep{maas2019facebook} . \footnote{This work leverages Facebooks internal survey infrastructure, details can be found in \citet{schneider_future_nodate}. Other projects that have employed the Facebook survey infrastructure include \citet{feehan2019using} in Demography, a longitudinal survey of small and medium business for the World Bank \citep{alekseev2020effects} and the Facebook COVID-19 Symptoms Survey \citep{kreuter2020partnering}. See \cite{kreuter2020partnering} for a discussion of working with Facebook on the Symptoms survey and working with internal survey infrastructure in general.} Rapid surveys on a platform such as Facebook provide a novel way of reaching individuals in situations that would otherwise render them prohibitively expensive or impractical to reach, and allow for high-quality demographic estimates in otherwise adverse circumstances. 

%This work can likewise provide a method of validating geo-location based methods like those employed by Facebook's Data for Good program. Researchers have used mobility data from cell phones and other electronic devices to characterize both short-term and long-term displacement after a disaster \citep{gething2011can}; however, this technique has often been limited by an inability to pair mobility data with key additional information.  We propose pairing such data with survey research to increase their usefulness.  In particular, many potential hypotheses could be explored if richer contextual information were available including but not limited to the household structure of displaced persons, the nature of locations to which displaced persons migrate (e.g. identification as a home of relatives) and the methods people use to relocate \citep{frankenberg2014demography}. 

 %From September 2019 to March 2020, Australia experienced one of the worst bushfires in modern history \citep{kganyago2020assessment}. Over this period it is estimated that 186,000 square kilometers were burned and 5,900 building were destroyed. This included more than three thousand homes \citep{filkov2020impact} and resulted in the displacement of tens of thousands of Australians. To better understand the economic and demographic effects of this disaster in Australia, we conducted a survey of Facebook users who could have been directly affected by the bushfires.\footnote{\citet{20192020AUSTRALIANBUSHFIRES} (IDMC) has attempted to estimate the economic and demographic effects of the Australia Bushfires using the data in this article as well as other data sources.  Specifically, IDMC found that  cost between \$44 million and \$52 million due to population displacement during and after the Bushfires.}  This, when combined with mobility estimates provided by the Data for Good program, could allow us to refine estimates derived from mobility data \citep{maas2019facebook} and to address hypotheses around how displacement affected people and households in the region -- information that cannot be obtained from observational migration data alone.  
 
%Conducting surveys from traditional sampling frames after a natural disaster is incredibly difficult and expensive \citep{sastry2009tracing}. This work looks to mitigate some of these issues by accessing a sampling frame that is more robust to displacement of potential respondents. By taking a random sample of Facebook users who were located in the disaster region before the disaster hit we are able to survey both those who are currently in the area and those who continue to be displaced or evacuated from the disaster. \footnote{This survey occurs two months after the disaster events under study.} 


%Specifically, we leverage Facebook's account data to build a stratified sample of respondents for our survey of displaced and evacuated individuals from the \emph{Green Wattle Creek Fire} in Eastern New South Wales and the \emph{Cudlee Creek Fire} in Adelaide Hills, South Australia (Figure~\ref{fig:survey_location}) bushfires in Australia. To do this we sample users who have geo-location data and meet the same home location criterion used by Facebook's Disaster Maps \citep{maas2019facebook} and a random sample of users who could have been in the region based on an internal Facebook analysis to guarantee representativeness of the population. 

%This resulting sample that is metaphorically similar to a hypothetical address based sample which was capable of following respondents after they were displaced, where instead of addresses we are following Facebook accounts.  Our estimates of displacements caused by these fires are broadly consistent with other findings, suggesting our novel frame is providing accurate data. Comparing total estimates of those displaced in Adelaide Hills, South Australia area due to the Cudlee  Creek  Fire we find 17,973 (17,741,18,205) people are displace at more than one night from January to February, 2020 which is close to estimates provided by IDMC \citep{20192020AUSTRALIANBUSHFIRES}. 


%The International Displaced Monitoring Centre \cite{20192020AUSTRALIANBUSHFIRES} estimates about 17,000 people were displaced January to February in the Adelaide Hills, South Australia from the Australian Red Cross data. For comparison, if you use our survey to estimate the number of people displaced we find that our survey would estimate that 17,973 (17,741,18,205) people were displaced from January to February for at least one night in the Adelaide Hills, South Australia.  A larger discussion on this sample follows in the Methodology section.

%In this study we partner with Facebook's Data for Good program to address the above limitations of post-disaster displacement surveys.  The Data for Good program has already used mobility data to develop an approach that both identifies migration and relocation after disasters \citep{maas2019facebook} and provides real-time information about displacement to non-governmental organizations (NGOs). In this study we extend their work by incorporating additional demographic and contextual information collected via a rapid-deployment survey following a disaster.  Rapid surveys on a platform such as Facebook provide a novel way of reaching individuals in situations that would otherwise render them prohibitively expensive or impractical to reach, and allow for high-quality demographic estimates in otherwise adverse circumstances. 

%This research provides two major contributions to the literature on demography and disasters: (1) a novel data collection strategy that can be paired with autmated geo-spatial methods for estimating displacement and displacement characteristics; and 2) provides data the displacement and demographics of Australians two months after the 2019 Australia bushfires. 

%This article is laid out in the following manner: (1) a brief overview of the social science of evacuation behavior to motivate the core set of research questions; (2) a review of the innovations related to our methodology; (3) a review the survey sample and comparison to the general Australian Facebook population and the general Australian population; (4) an analysis of the survey associated with our research questions (5) a discussion of policy implications and areas for future research.




%social  science  literature  on  evacuation  behavior.

%thorough review of the social  science  literature  on  evacuation  behavior.   (Note  that  this  is  not  the  same as  migration  behavior  since  it  is  temporary  mobility.) 

%The  literature  review  and discussion should clearly identify the contribution of the study and how it builds on the existing literature.

%Third, since Facebook data are a new source of data for studying evacuation behavior in response to rapid onset natural disasters it is important that you thoroughly discuss the  method  of  data  collection,  its  strengths  and  weaknesses,  and  how  it  comparesto  other  data  sources.   If  the  innovative  data  is  one  of  the  contributions  of  this manuscript, this should be emphasized alongside the empirical results.


% Specific Literature Review Suggestions 

%%%% Reviewer 1
% L131 There is more recent studies.  See Martin et al.  2020 or Alexander et al.(2019).  Mart ́ın, Y., Cutter, S. L., Li, Z., Emrich, C. T.,  Mitchell, J. T. (2020).Using geotagged tweets to track population movements to and from Puerto Ricoafter Hurricane Maria.  Population and Environment, 1-24.
% Alexander, M., Zagheni, E.,  Polimis, K. (2019).  The impact of Hurricane Mariaon out-migration from Puerto Rico:  Evidence from Facebook data.

%L144: Claim about climate change increasing natural disasters needs a reference.Also, climate change could be increasing the frequency and intensity of naturalHAZARDS,  disasters  have  a  human  component.   Disasters  can  increase  dueto  occupation  of  hazardous  land  more  than  the  increase  of  hazards.   Please,revise this duality (hazard/disaster) throughout the manuscript to make sure itis accurate.

% L208:   Again,  the  authors  are  missing  out  platforms  such  as  Twitter,  whichhave been useful to identify pre and post-disaster population movements andidentify  gender  differences  in  the  response:  Mart ́ın,  Y.,  Cutter,  S.  L.,   Li,  Z.(2020).  Bridging twitter and survey data for evacuation assessment of HurricaneMatthew and Hurricane Irma.  Natural hazards review, 21(2), 04020003

%%%%%%% Reviewer 2
%Similarly, the authors observe that the vast majority of people who evacuate do soby  car.   Here  an  examination  of  Census  data  on  lack  of  access  to  vehicles  mightpoint to important policy decisions about assisted evacuation for households withoutvehicles.   For  literature  on  carless  evacuation  planning  see  John  Renne,  ThomasSanchez  and  Todd  Litman.   “Carless  and  Special  Needs  Evacuation  Planning:   ALiterature Review,” Journal of Planning Literature,  Vol.  26,  No.  4,  pp.  420-431,2011.

% The authors’ focus primarily on differences by gender, but the paper would benefitfrom additional analyses of difference in evacuation experience and behavior by otherdemographic variables such as income, educational attainment, and presence of chil-dren in a household.  In particular, it would be interesting to know if households withchildren are less likely to return to areas that evacuees consider unsafe following adisaster.  This could inform policy decisions about the reopening of schools after adisaster.

%The authors asked how many nights a household was displaced and found that 55percent of their sample was evacuated for 7 nights or more.  But the authors analyzedresponses based on one night, one to three nights or more than three night, based onliterature by Maas et al 2019.  The authors may want to review additional literatureor use their own data to identify longer displacement periods that more meaningfullydefine long term, disruptive displacement.


%%%%%%%%%%%
%%% Reviewer 3
%%%%%%%%%%%
%Your literature review section could do more work to explore what migration and dis-aster researchers have found regarding your specific research questions (rather thanjust general findings of environment-related displacement).  How do previous findingsinform your hypotheses?  If these research questions have never been examined,  itwould be worthwhile to state that.  Additionally, disaster research often specifies adifference in timescale that differentiates evacuation versus longer-term migration.  Ithink outlining a clearer framework around the temporal language you use (evacua-tion, migration, displacement, etc.)  would strengthen the paper.

% Lines  42  –  50:  These  examples  don’t  really  illustrate  why  understanding  de-mographic heterogeneity is important – there are other works on disaster dis-placement  that  more  explicitly  examine  differential  mobility  outcomes  acrossdifferent demographic groups.  For example, there is a good amount of this typeof research around Hurricane Katrina.

% Line 97:  Consider renaming the “Literature Review” section to something moretopic-specific.
% The section on “Disasters and Demography” could be sharpened by honing inon migration literature specifically;  I don’t think you need to gesture towardsfertility/mortality/health  if  you  aren’t  researching  these  topics.   This  sectionfeels  a  bit  thin,  and  could  be  especially  improved  by  discussing  literature  ongender and displacement, since that is one of your core areas of investigation.



%%%%%%%%
%% Discussion of population Facebook
%%%%%%%%%
%% Reviewer 2
%While the sampling methodology appears to yield a representative sample of Facebookusers, to ensure that findings are suitable for policy decision making, the paper wouldbenefit  from  a  bit  more  discussion  of  how  Facebook  users  differ  from  the  overallpopulation.   While  the  age  distribution  does  not  differ  from  the  full  population,Facebook users may differ from the overall population in other ways that would bevery important to equitable policy making.  Specifically,  Facebook users may havehigher  incomes  and  greater  educational  attainment.   If  so,  this  limitation  of  theFacebook  user  universe  should  be  understood  when  using  Facebook  user  data  toinform policy decisions

%% Reviewer 3
% It would be useful to include a discussion of which populations Facebook’s mobilitydata capture, and which they do not.  Who doesn’t use Facebook, or who opts out ofLocation History and would therefore be excluded from your datasets?  This analysiswould help other migration scholars understand how Facebook’s data offerings differfrom more widely used migration data sources.  You have a few lines in the end ofthe paper (488-490), but this discussion would benefit from being much earlier in thepaper and in greater depth

%This online appendix contains a flow diagram of the FB Displacement %Survey (Figure~\ref{fig:flow}) and the questionnaire. 

%\begin{figure}[h]
%    \centering
%  \includegraphics[width=.9\linewidth]{graphics/Survey-Flows-for-%Paper.pdf}
%\caption{Diagram of the survey flow. Numbers give the approximate number of people who answered the question.}
%\label{fig:flow}       
%\end{figure}

%\includegraphics[width=1.3\linewidth]{survey/au_bushfire_survey1.pdf}

%\includegraphics[width=1.3\linewidth]{survey/au_bushfire_survey2.pdf}

%\includegraphics[width=1.3\linewidth]{survey/au_bushfire_survey3.pdf}

%\includegraphics[width=1.3\linewidth]{survey/au_bushfire_survey4.pdf}

%\includegraphics[width=1.3\linewidth]{survey/au_bushfire_survey5.pdf}

%\includegraphics[width=1.3\linewidth]{survey/au_bushfire_survey6.pdf}



\begin{figure*}
  \centering
\begin{subfigure}[t]{0.45\textwidth}
    \centering
    \includegraphics[width=\linewidth]{graphics/Total_weights_q28_mask_access_by_gender.pdf} 
    \caption{Mask Access by Gender} \label{fig:masks1}
\end{subfigure}
\hfill
\begin{subfigure}[t]{0.45\textwidth}
    \centering
    \includegraphics[width=\linewidth]{graphics/Total_weights_q29_mask_knowledge_by_gender.pdf} 
    \caption{Mask Knowledge by Gender} \label{fig:masks2}
\end{subfigure}

\caption{Men are significantly more likely to report that they had access to N95 smoke masks during the Australian bushfires in December 2019, and that they can tell if a mask is effective.}
\label{fig:6}       
\end{figure*}
%

\begin{figure}

  \includegraphics[width=\linewidth]{graphics/Total_weights_q29_mask_knowledge_regression_no_interaction_with_mask_access_income_displacement.pdf}

\caption{Odds ratio for not knowing whether a mask is effective, compared to knowing, adjusted for age, gender, income, mask access, and duration displaced.  People without mask access have 5.5 times the odds of not knowing whether a mask is effective; controlling for that, women have 1.6 times the odds of not knowing. Values presented in Table \ref{Total_weights_q29_mask_knowledge_regression_no_interaction_with_mask_access_income_displacement}.}
\label{fig:7}       
\end{figure}

\begin{table}
\begin{longtable}{llrlll}
  \hline
Response & Covariate & Odds Ratio & 95\% CI & P Value & Significance \\ 
  \hline
No & Gender: Male & 1.00 &  &  &  \\ 
  No & Gender: Female & 1.57 & (1.51, 1.6) & 0.000 & *** \\ 
  No & Gender: Prefer Not to Say & 1.00 & (NaN, NaN) & NaN &  \\ 
  No & Age: 20-29 & 1.06 & (1.00, 1.1) & 0.057 & . \\ 
  No & Age: 30-39 & 1.00 &  &  &  \\ 
  No & Age: 40-49 & 0.89 & (0.84, 0.9) & 0.000 & *** \\ 
  No & Age: 50-59 & 0.84 & (0.79, 0.9) & 0.000 & *** \\ 
  No & Age: 60-69 & 0.97 & (0.91, 1.0) & 0.464 &   \\ 
  No & Age: 70+ & 1.43 & (1.31, 1.6) & 0.000 & *** \\ 
  No & Age: Prefer Not to Say & 1.21 & (1.06, 1.4) & 0.004 & ** \\ 
  No & Education: Elementary & 1.21 & (1.00, 1.5) & 0.056 & . \\ 
  No & Education: Junior High & 1.51 & (1.30, 1.7) & 0.000 & *** \\ 
  No & Education: High School & 1.19 & (1.10, 1.3) & 0.000 & *** \\ 
  No & Education: Community College & 1.02 & (0.95, 1.1) & 0.550 &   \\ 
  No & Education: University & 1.00 &  &  &  \\ 
  No & Education: Graduate School & 0.99 & (0.90, 1.1) & 0.764 &   \\ 
  No & Education: Prefer Not to Say & 1.18 & (1.07, 1.3) & 0.001 & *** \\ 
  No & Household\_head: Yes & 1.00 &  &  &  \\ 
  No & Household\_head: No & 1.21 & (1.16, 1.3) & 0.000 & *** \\ 
  No & Mask\_access: Yes & 1.00 &  &  &  \\ 
  No & Mask\_access: No & 5.45 & (5.24, 5.7) & 0.000 & *** \\ 
   \hline
\hline
\caption{Mask knowledge, compared to ``yes"; relative to university-educated men, aged 30-39, head of household, with mask access based on the model with main effects for age, gender, education, and head of household with no interactions} 
\label{Total_weights_q29_mask_knowledge_regression_no_interaction_with_mask_access}
\end{longtable}
\end{table}

 \begin{figure*}[!htb]
        \includegraphics[width=0.8\linewidth]{graphics/Total_weights_q28_mask_access_regression_no_interaction_with_income_displacement.pdf} 
        \caption{Mask access, compared to ``yes"; relative to men, aged 30-39, income less than \$3,200 head of household, not displaced based on model with main effects for age, gender, income, head of household, and duration displaced with no interactions.} \label{fig:Total_weights_q28_mask_access_regression_no_interaction_with_income_displacement1}
    \label{fig:Total_weights_q28_mask_access_regression_no_interaction_with_income_displacement}
\end{figure*}
